Deleting and Testing Forbidden Patterns in Multi-Dimensional Arrays

Understanding the local behaviour of structured multi-dimensional data is a fundamental problem in various areas of computer science. As the amount of data is often huge, it is desirable to obtain sublinear time algorithms, and specifically property testers, to understand local properties of the data. We focus on the natural local problem of testing pattern freeness: given a large $d$-dimensional array $A$ and a fixed $d$-dimensional pattern $P$ over a finite alphabet, we say that $A$ is $P$-free if it does not contain a copy of the forbidden pattern $P$ as a consecutive subarray. The distance of $A$ to $P$-freeness is the fraction of entries of $A$ that need to be modified to make it $P$-free. For any $\epsilon \in [0,1]$ and any large enough pattern $P$ over any alphabet, other than a very small set of exceptional patterns, we design a tolerant tester that distinguishes between the case that the distance is at least $\epsilon$ and the case that it is at most $a_d \epsilon$, with query complexity and running time $c_d \epsilon^{-1}$, where $a_d < 1$ and $c_d$ depend only on $d$. To analyze the testers we establish several combinatorial results, including the following $d$-dimensional modification lemma, which might be of independent interest: for any large enough pattern $P$ over any alphabet (excluding a small set of exceptional patterns for the binary case), and any array $A$ containing a copy of $P$, one can delete this copy by modifying one of its locations without creating new $P$-copies in $A$. Our results address an open question of Fischer and Newman, who asked whether there exist efficient testers for properties related to tight substructures in multi-dimensional structured data. They serve as a first step towards a general understanding of local properties of multi-dimensional arrays, as any such property can be characterized by a fixed family of forbidden patterns.

==> distance_vs_hitting_highD.tex <==
\subsection{Deletion number versus hitting number}\label{sec:distance_vs_hitting}
Here we prove a useful relation between the distance and the hitting number, as given in Lemma~\ref{lem:hitting_set_2D} below, which is proved by analyzing a procedure that uses the modification lemma to remove all copies of $P$ from $M$.

\begin{lemma}\label{lem:hitting_set_2D}
\textnormal{\textbf{[relation between distance and hitting number]}}
Let $P$ be a removable $(k,d)$-array over an alphabet $\Gamma$, and let $A$ be an $(n,d)$-array over $\Gamma$. Let $\alpha_d = 4^d + 2^d$. It holds that
\[
h_P(A) \leq d_P(A) \leq \alpha_d h_P(A) \leq \alpha_d k^{-d}.
\]
\end{lemma}

\begin{proof}
The first inequality follows from the fact that one needs to modify at least one entry in any $P$-copy in $A$. 
For the third inequality, note that the set $\{(x_1, \ldots, x_d) \in [k]^d : \forall 1 \leq i \leq d,\  x_i \equiv k-1 (\text{mod }{k})\}$ is a set of size $[n/k]^d$ that hits all $k \times \ldots \times k$ consecutive subarrays of $A$, and in particular all $P$-copies. 
It remains to prove that $d_P(A) \leq \alpha_d h_P(A)$. 
We may assume that the alphabet $\Gamma$ is binary by applying the standard reduction from non-binary to binary alphabets presented in Section \ref{sec.modification.lemmas}.

We present a procedure on the array $A$ that makes it $P$-free by sequentially flipping bits in it. 
In what follows, we will say that the \emph{center} of a $(k,d)$ matrix lies in location $(\lfloor k/2 \rfloor, \ldots, \lfloor k/2 \rfloor)$ in the matrix.
Let $\cal \mathcal{P}$ be the set of all $P$-copies \emph{before} $A$ is modified.
In Phase 1, the procedure "destroys" all $P$-copies in $\mathcal{P}$ by flipping central bits of a subset of the original $P$-copies in $A$, which is chosen in a greedy manner. However, these bit flips might create new $P$-copies in $M$, which are removed in Phase 2 using the modification lemma.
The procedure maintains sets ${\cal A}, {\cal B}$ that contain the bits flipped in phases 1,2 respectively.
%Different from the 1D procedure, \emph{new} pattern occurrences might be created as a result of the sequential flipping of matrix bits. We therefore differentiate between the \emph{original} occurrences and those that are \emph{created} during the procedure and did not exist in the original matrix $M$. In Phase A, the procedure iteratively collects a set ${\cal O}$ of original occurrences, which we will later show to be $1/2$-independent. After an occurrence is added to ${\cal O}$ one of its bits is flipped. We keep iterating until no original occurrences of $P$ remain. Note that as a result of the flipping, new occurrences might be created. In Phase B, we will continue flipping bits, one per remaining (newly created) occurrence \emph{without} creating new ones, until $M$ becomes $P$-free.

\begin{itemize}\vspace{-5pt}
  \item Let ${\cal P}$ be the set of all $P$-copies in $A$, ${\cal N} \leftarrow \phi$ ${\cal A} \leftarrow\phi$, ${\cal B}\leftarrow\phi$.% , $NA=\phi$
%  \item Let $OCC$ be the set of original occurrences
%  \item Repeat as long as ${\cal O}<(\epsilon n)/100\;$ \footnote{No attempt has been made to optimize the constants}
  \item \textbf{Phase 1: }While ${\cal P} \neq \phi$
  \begin{itemize}
    \item Pick $Q \in {\cal P}$ arbitrarily.
    \item Flip $A_x$ where $x$ is the center of $Q$.
    \item Add $Q$ to ${\cal A}$ and remove all $P$-copies containing $x$ from ${\cal P}$.
    \item Add all $P$-copies \emph{created} by flipping $A_x$ to $\cal N$.
    \end{itemize}
  \item \textbf{Phase 2: }While ${\cal N} \neq \phi$
  \begin{itemize}
    \item Pick $Q \in {\cal N}$ arbitrarily.
    \item Pick a location $x$ in $Q$ whose flipping does not create new $P$-copies in $A$ (exists by modification lemma).
    \item Flip the bit $A_x$ and add $x$ to ${\cal B}$.
  \end{itemize}
\end{itemize}
For the analysis of the procedure, we say that two $P$-copies $Q,Q'$ in $A$ whose starting points are $x = (x_1, \ldots, x_d), y = (y_1, \ldots, y_d) \in [n]^d$ respectively are \emph{$1/2$-independent} if $|x_i - y_i| \geq k/2$ for some $1 \leq i \leq d$.
Note that $1/2$-independence is a symmetric relation.
A set of $P$-copies is $1/2$-independent if all pairs of copies in it are $1/2$-independent. Denote by $i_{P}(A)$ the maximal size of a $1/2$-indpendent set in $A$, divided by $n^d$.

For $Q$ and $Q'$ as above, if $Q'$ does not contain the center of $Q$ then $Q,Q'$ are $1/2$-independent, as 
there is some $1 \leq i \leq d$ for which either $y_i < x_i + \lfloor k/2 \rfloor - (k-1) \leq x_i - k/2 + 1$ or $y_i > x_i + \lfloor k / 2 \rfloor \geq x_i + k/2 -1$.
In both cases $|y_i - x_i| \geq k/2$, implying the $1/2$-independence.
Therefore the set ${\cal A}$ generated by the procedure is $1/2$-independent: if $Q, Q' \in {\cal A}$ are two different $P$-copies and $Q$ was added to $\cal A$ before $Q'$, then $Q'$ does not contain the center of $Q'$, so $Q$ and $Q'$ are $1/2$-independent. 
Using the following claims, it is not hard finish the proof of the lemma.%, as they imply that $|{\cal A}| + |{\cal B}| \leq \alpha_d n^d d_P(A)$.
\begin{claim}
\label{clm:independece_hitting}
$i_P(A) \leq 2^d h_P(A)$.
\end{claim}
The proof of Claim \ref{clm:independece_hitting} will be given later.
For what follows, we say that
$P$ has a \emph{cycle} of size $t=(t_1,\ldots,t_d)\in\mathbb{Z}^d$, if $P_x=P_y$ for every pair of locations $x=(x_1,\ldots,x_d),y=(y_1,\ldots,j_d)\in[k]^d$ such that $x_i\equiv y_i \Mod{|t_i|}$ $\forall i\in[d]$.
The following claim is straightforward to verify.
\begin{claim}\label{obs:overlap_to_cyclic_2D}
\textnormal{{[Shifted occurrences imply a cyclic pattern]}}
If $M$ contains two overlapping occurrences of $A$, at a relative offset of $t\in\mathbb{Z}^d$, then $P$ has a cycle of size $t$.
\end{claim}

\begin{claim}\label{clm:Bit_flip_no_new_occurrences_2D}
\textnormal{{[Central bit flip creates few new occurrences]}}
Flipping the central bit of a $P$-occurrence in $A$ creates at most $2^d$ new occurrences of $P$ in $A$.
\end{claim}

We first show how to use these claims to finish the proof.
Consider the sets $\mathcal{A}, \mathcal{B}$ after the procedure ends. 
The procedure flips $|{\cal A}| + |{\cal B}|$ bits in $A$, so $|{\cal A}| + |{\cal B}| \geq d_P(A) n^d$.  
On the other hand, $|\mathcal{A}| \leq i_P(A) n^d \leq (2n)^d h_P(A)$ as $\cal A$ is $1/2$-independent.
Claim \ref{clm:Bit_flip_no_new_occurrences_2D} now implies that $|{\cal B}| \leq 2^d|{\cal A}|$, and we get that
\[
n^d d_P(A) \leq |{\cal A}| + |{\cal B}| \leq (2^d+1)|\mathcal{A}| \leq \alpha_d  n^d h_P(A)
\]
Dividing by $n^d$ yields the desired inequality. We now prove the claims.
\begin{proof}[Proof of Claim \ref{clm:independece_hitting}]
Let $\cal S$ be a $1/2$-independent set of $P$-copies in $A$, which is of size $i_P(A)$. 
We will show that no point in $[n]^d$ is contained in more than $2^d$ copies from $S$, implying that to hit all copies of $P$ in $A$
(and in particular, all copies of $P$ in $\cal S$) we will need at least $|{\cal S}| / 2^d = i_P(A) / 2^d$ entries.

Suppose to the contrary that there are $2^d + 1$ copies from $\cal S$ that contain the point $x = (x_1, \ldots, x_d) \in [n]^d$.
we will say that a copy from $\cal S$ containing $x$ is $i$-lower if $k/2 \leq x_i - y_i < k$
and $i$-higher if $0 \leq x_i - y_i < k/2$ (note that $0 \leq x_i - y_i < k$ must hold). 
Therefore, there exist two copies $Q, Q' \in {\cal S}$ containing $x$, starting at $(y_1, \ldots, y_d)$ and $(y'_1, \ldots, y'_d)$ respectively, such that for any $1 \leq i \leq d$, $Q$ is $i$-higher ($i$-lower)
\emph{if and only if} $Q'$ is $i$-higher ($i$-lower respectively). 
But then, for any $i$, either $0 \leq y_i, y'_i < k/2$ or $k/2 \leq y_i, y'_i < k$, implying that $|y_i - y'_i| < k/2$, thus contradicting the fact that $\cal S$ is $1/2$-independent.
\end{proof}
\begin{proof}[Proof of Claim \ref{clm:Bit_flip_no_new_occurrences_2D}]
Assume that more than $2^d$ new occurrences are created. Since these occurrences overlap (at the bit flip location),the same argument as in Claim \ref{clm:independece_hitting} implies that there must be two of them, $P_1$ and $P_2$, that are shifted (one from the other) by some vector $t\in\mathbb{Z}^d$, where $|t_i|<k/2$ $\forall i\in[d]$.

By Claim \ref{obs:overlap_to_cyclic_2D}, $P$ (and hence also $P_1$ and $P_2$) has a cycle of size $t$.
Let $x$ be the point in $M$ of the (central) flipped bit in $P_0$ and consider the point $x'=x+t$, which is also in $P_0$, since $|t_i|< k/2$ $\forall 1\le i \le k$. The occurrence $P_2$ overlaps both locations $x$ and $x'$ (since both new occurrences $P_1$ and $P_2$ overlap the bit flip location $x$ and $P_2$ is shifted by $t$ from $P_1$, which overlaps $x$).

On one hand we have $M_x=M_{x'}$ (before the bit flip), since both locations belong to $P_0$, which has a cycle of size $t$. On the other hand, $M_x\neq M_{x'}$, since these locations both belong to $P_2$ and must be equal \emph{after} flipping $M_x$ as $P_2$ has a cycle length of $t$. This leads to a contradiction.
\end{proof}
\end{proof}


==> higher_dimensions.tex <==
\section{The multi-dimensional case}
\label{sec.2-dimension}
In this section we devise a distance approximation algorithm and a tolerant tester
for pattern freeness in two and higher dimensions when the pattern is removable (i.e.\@ non-almost-homogeneous and large enough).
We start by showing that when $P$ is removable,
the $P$-hitting number $h_P(A)$ of $A$ approximates the distance to $P$-freeness up to
a multiplicative constant that depends only on the dimension $d$, as is shown in Subsection \ref{subsec.distance_vs_hitting}. We then show that approximating the hitting number $h_P(A)$ with
small additive and multiplicative errors can be done very efficiently, similarly to what was shown in the 
one-dimensional case.
We conclude by devising a tolerant tester that has multiplicative tolerance that depands only on $d$,
and whose query complexity and running time are optimal.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Distance versus hitting (appears as a subsection)
\input{distance_vs_hitting_highD}\label{subsec.distance_vs_hitting}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Omri - Approximation and testing should go here..
\subsection{Tolerant testing and approximation}
\label{subsec.test_highD}
Deriving a distance approximation algorithm and a tolerant tester for $P$-freeness is quite similar to the one dimensional case.
We will describe how to approximate the hitting number $h_P(A)$ up to a multiplicative $(1+\tau)^d$ factor with number of queries and running time of $O_{\tau}(\epsilon^{-1})$, where the constant depends only on $\tau$. 
By Lemma \ref{lem:hitting_set_2D}, this yields the desired approximation to the deleting number $d_P(A)$, whose factor is $\alpha_d (1+\tau)^d = (4+4\tau)^d + (2+2\tau)^d$ (and in particular, does not depend on $k$ or $n$).
The main statements are as follows.

\begin{theorem}
\label{thm:approx_highD}
Let $P$ be a removable $(k,d)$-array and fix constants $0 < \tau \leq 1,0 \leq \delta \leq 1/k$. 
Let $h_1, h_2:[0,1] \to [0,1]$ be defined as $h_1(\epsilon) = (1-\tau)^d \alpha_d^{-1}\epsilon - \delta$  and $h_2(\epsilon) = \epsilon + \delta$.
There exists an $(h_1, h_2)$-distance approximation algorithm for $P$-freeness
making at most $\gamma / k^d \tau^d \delta^2$ queries, where $\gamma > 0$ is an absolute constant, and has running time 
$\zeta_\tau / k^d \delta^2$ where $\zeta_\tau$ is a constant that depends only on $\tau$.
%making at most $\alpha k\epsilon (1/k-\epsilon) / \tau \delta^2 \leq \alpha \epsilon / \tau \delta^2$ queries, where $\alpha > 0$ is an absolute constant.
\end{theorem}


\begin{theorem}
\label{thm:test_highD}
Fix $0 < \tau \leq 1$ and let $P$ be a removable $(k,d)$-array. For any $0 < \epsilon \leq 1$ there exists a $((1-\tau)^d \alpha_{d}^{-1}\epsilon, \epsilon)$-tolerant tester making $C_\tau \epsilon^{-1}$ queries, where $C_\tau = O(1 / \tau^d (1 - (1-\tau)^d)^2)$.
The running time is $C'_\tau \epsilon^{-1}$ where $C'_\tau$ depends only on $\tau$.
\end{theorem}

As the technical details here are very similar to those in the 1D case, we will only sketch the main ideas. 
Take $\beta = 2 / \tau$.
Let $A$ be an $(n,d)$-array where we may assume that $n \geq \beta k$ for a suitable choice of $C$.
Again, the strategy is to take $t$ (to be determined) independent samples of blocks of size $\beta k \times \ldots \times \beta k$
and compute the hitting number of each sampled block.
Note that (as opposed to the one-dimensional case), computing the minimal hitting set is generally an $NP$-complete problem, but 
since the hitting number of each of these blocks is at most $\beta^d = \Theta(\tau^{-d})$, here we may compute it
with running time that depends only on $\tau$ and $d$.
As in the 1D case, the expected relative hitting number $\mu$ of a sampled block satisfies $(1-\tau)^d h_P(A) = (1-2/\beta)^d h_P(A) \leq \mu \leq h_P(A)$.
The variance of the hitting number for a single sample is no bigger than $k^d (1/k^d - \mu)^2 + (1 - k^d \mu)\mu^2 = \mu(1/k^d-\mu) \leq \mu / k^d$, so for $t$ samples it is $O(h_P(A) / k^d t)$.
To get additive error of at most $\delta$ with constant probability, we may have (by Chebyshev inequality) $h_P(A) / k^d t = \Theta(\delta^2)$,
or $t = \Theta(h_P(A) / k^d \delta^2)$.

Therefore, for an approximation algorithm (in which we don't know $h_P(A)$ in advance, though we have an upper bound of $h_P(A) \leq 1 / k^d$), $t = \Theta(k^{-2d} \delta^{-2})$ sampled blocks are enough,
and the total number of samples is $O(1 / k^d \tau^d \delta^2)$.
For a $((1-\tau)^d\epsilon, \epsilon)$-tolerant tester for the hitting number (which translates to a $((1-\tau)^d \alpha_d^{-1} \epsilon, \epsilon)$-tolerant tester for the deletion number), as observed in the 1D case, when deciding on the number of samples we may assume that $h_P(A) = \epsilon$ and pick $\delta  = \Theta((1-(1-\tau)^d) \epsilon)$ , so $t = \Theta(\epsilon / k^d \delta^2) = \Theta(1 / k^d (1 - (1-\tau)^d)^2 \epsilon)$ sampled block suffice. Since each block is of size $\Theta(k^d / \tau^d)$, the total number of queries is $O(C_\tau \epsilon^{-1})$ where $C_\tau = 1 / \tau^d (1 - (1 - \tau)^d)^2$, while the running time is $C'_\tau \epsilon^{-1}$, where $C'_\tau$ depends on the time required to compute the hitting number in a single sampled block.

==> one_dimension.tex <==
\section{The one-dimensional case}
In this section we consider the problems of computing and approximating the
distance to $P$-freeness in the one dimensional case, when $P$ is removable (i.e.\@ not almost homogeneous).
The case where $P$ is almost homogeneous is settled in Appendix \ref{sec:almost_homo}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Minimal Deletion Set versus Minimal Hitting Set}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We present an optimal (linear time) algorithm for the exact computation of the distance $d_P(S)$ of a string $S$ from being $P$-free for a removable pattern $P$. The core of the proof is a surprising combinatorial characterization of the deletion number: it shows that one can construct a hitting set 
which is also a deletion set. The proof %of Theorem \ref{thm.1D.minDeleting.equals.minHitting.Plus.Exact} 
appears in Appendix~\ref{append.sec.min.hit.min.dist}.
\begin{theorem}
[$d_P(S)$ equals $h_P(S)$; Linear time computation of $d_P(S)$]
\label{thm.1D.minDeleting.equals.minHitting.Plus.Exact}
For a binary string $S$ of length $n$ and a binary pattern $P$ of length $k$ that is removable, the deletion number $d_P(S)$ equals $h_P(S)$ and can be computed in time $O(n+k)$ and space $O(m)$.
\end{theorem}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tolerant Testing of Pattern Freeness}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\label{sec.1-dimension}
%Following the reduction of the non-binary case to the binary case that was shown in the beginning of Theorem \ref{thm:modification},
%it will be enough to consider binary strings.
%For a string $S$, let $d_P(S)$ denote the absolute distance of $S$ from $P$-freeness and let $\delta_P(S) = d_P(S) / n$ denote the relative distance.
%Also let the \emph{hitting number} $h_P(S)$ denote the minimal size of a set $A$ of entries of $S$ such that any $P$-copy in $S$ contains some entry from $A$.
Consider a string $S$ of length $n$ and a removable string $P$ of length $k$.
If $S$ is $\epsilon$-far from $P$-freeness then (by the 1D modification lemma) there are at least $\epsilon n$ copies of $P$,
suggesting the following naive way to devise a tester for $P$-freeness in this case:
make $t = \Theta(\epsilon^{-1})$ independent block samples in $S$, each of length $k$, and accept if and only if no $P$-copy was found.
However, this tester has query complexity $O(\epsilon^{-1}k)$ that depends on $k$, and is not very tolerant: it has multiplicative tolerance of $k$. 
In what follows, we describe a tester that overcomes these two problem (and can also serve as a distance approximation algorithm).
For a constant $\tau > 0$, we present a tester with running time $O_\tau(\epsilon^{-1})$, which is optimal (up to the dependence on $\tau$),
and a multiplicative tolerance of $1 + \tau$. 

We start by presenting the distance approximation algorithm for $P$-freeness.
The approximation here has both additive and multiplicative errors.
\begin{theorem}%[\emph Testing in $1D$]
\label{thm:approx1D}
Let $P$ be a removable string of length $k$ and fix constants $0 < \tau < 1, 0 < \delta < 1/k$.
Let $h_1, h_2:[0,1] \to [0,1]$ be defined as $h_1(\epsilon) = (1-\tau)\epsilon - \delta$  and $h_2(\epsilon) = \epsilon + \delta$.
There exists an $(h_1, h_2)$-distance approximation algorithm for $P$-freeness
with query complexity and running time of $O(1/ k \tau \delta^2)$.
%making at most $\alpha k\epsilon (1/k-\epsilon) / \tau \delta^2 \leq \alpha \epsilon / \tau \delta^2$ queries, where $\alpha > 0$ is an absolute constant.
\end{theorem}
Note that $d_P(S) = h_P(S) \leq 1/k$ always holds, so having an additive error parameter of $\delta \geq 1/k$ is pointless.
The proof of
Theorem \ref{thm:approx1D} can be adapted to derive $(\epsilon_1, \epsilon_2)$-tolerant testers
for any $0 \leq \epsilon_1 < \epsilon_2 \leq 1$.
\begin{theorem}
\label{thm:test_1D}
Let $P$ be a removable string of length $k$ and let $0 \leq \epsilon_1 < \epsilon_2 \leq 1$. There exists an $(\epsilon_1, \epsilon_2)$-tolerant tester
whose number of queries and running time are $O(\epsilon_2^2 / (\epsilon_2 - \epsilon_1)^3)$ where the constant term does not depend on $k$.
\end{theorem}
It is not clear whether this upper bound is tight in general.
However, for the important special case of tolerant testers with multiplicative tolerance of $1 + \tau$,
where $\tau > 0$ is a constant, the above tester is optimal (up to a multiplicative constant that depends on $\tau$), as is
shown by taking $\epsilon_2 = \epsilon$ and $\epsilon_1 = (1-\tau)\epsilon$ in Theorem \ref{thm:test_1D}.
\begin{corollary}
Fix $0 < \tau < 1$. For any $0 < \epsilon \leq 1$ there exists a $((1-\tau)\epsilon, \epsilon)$-tolerant tester
whose number of queries and running time are $O(\epsilon^{-1} \tau^{-3})$.
\end{corollary}
%
%
%Again, the running time of the above tester is optimal (up to a multiplicative constant).
%In particular, it does not depend on the length of the forbidden pattern $P$ or the tested string.
%We did not try to optimize the tolerance factor in the above statement.

\begin{proof}[Proof of Theorems \ref{thm:approx1D} and \ref{thm:test_1D}]
Let $S$ be a string of length $n \geq \beta k$, where $\beta = 3 / \tau$. Write $\epsilon = \delta_P(S)$
and let $H \subseteq [n]$ be a hitting set for $P$ in $S$ whose size is $\epsilon n$. That is, $H$ is a minimal set of locations that satisfies the following: if $S$ contains a copy of $P$ starting at location $l$, then
$\{l, \ldots, l+k-1\} \cap H \neq \phi$.

For $i \in [n]$ let $I_i$ denote the ``cyclic interval'' of length $\beta k$ starting at $i$. That is, if $i + \beta k > n$ then $I_i = \{i, \ldots, n\} \cup \{0, \ldots, i + \beta k - n - 1\}$ and otherwise $I_i = \{i, \ldots, i + \beta_k - 1\}$. %The left endpoint and the right endpoint of $I_i$ are $l_i = i$ and $r_i = (i + \beta k - 1) \mod{n}$, respectively.

Let the random variable $X$ denote the
size of the minimal hitting set $H_i$ for $P$ in the interval $I_i$, divided by $\beta k$, where $i \in [n]$ is chosen uniformly at random.
Note that $X$ is computable in time $O(\beta k)$, by Theorem \ref{thm.1D.minDeleting.equals.minHitting.Plus.Exac}.
Let $\mu$ and $\sigma^2$ denote the expectation and the variance of $X$, respectively.
By the minimality of $H_i$, we have that $|H_i| \leq |H \cap I_i|$ since the set in the RHS is a hitting set for $P$ with respect to the interval $I_i$.
Thus, $\mu \leq \mathbb{E}[|H \cap I_i|] / \beta k = \epsilon$.

Next we bound $\mu$ from below.
Since $H_i$ hits all $P$-copies that lie exclusively inside $I_i$, and by the minimality of $H$, we must have
$|H_i| > |H \cap I'_i|$ where $I'_i$ is the cyclic interval that starts in $i+k$ and ends in $(i + (\beta-1)k - 1) \mod{n}$.
Therefore, $\mu \geq \mathbb{E}[H \cap I'_i] / \beta k = (1-2/\beta) \epsilon \geq (1-\tau)\epsilon$.
To conclude, we have seen that $(1 - \tau)\epsilon \leq \mu \leq \epsilon$.

%On the other hand, note that $X = |H_i| \geq |H \cap S^i| - \zeta_L^i -\zeta_R^i \geq |H \cap S_i| - 2$ where $\zeta_L^i$ ($\zeta_R^i$) is an indicator variable
%whose value is $1$ if and only if the leftmost entry $S_i$ (respectively rightmost entry $S_{(i+\beta k - 1)\mod{n}}$) of $S^i$ participates in some $P$-copy in $S$. %This follows from the fact that if $H_i$ was smaller than that,
%This occurs only if the leftmost (rightmost) entry is within distance of less than $k$ to the closest element in $H$.% from the right side (left side resp.\@).
%Therefore, $\Pr(\zeta_L^i), \Pr(\zeta_R^i) \leq k \epsilon$, implying that $\mu \geq (\beta - 2) k \epsilon$. % (in particular, we require $\beta \geq 5$).
%Thus, $\mu / \beta k \epsilon \in [1-2/\beta, 1]$.

To compute the variance of $X$, note that $0 \leq X \leq 1/k$, as there exist $\beta$ entries in $I_i$ such that any subinterval of length $k$ in $I_i$ contains at least one of them. By convexity, the variance satisfies $\sigma^2 \leq k\mu (1/k - \mu)^2 + (1 - k\mu) (0 - \mu)^2 = \mu (1/k-\mu) \leq \epsilon / k$.

Now let $Y = \frac{1}{t}\sum_{j=1}^{t} X_j$ where the $X_j$ are independent copies of $X$ and $t$ will be determined later. Then $\mathbb{E}[Y] = \mu$ and $\text{Var}(Y) = \sigma^2 / t  \leq \epsilon / k t$.

%Our approximation algorithm simply estimates $Y$ by making $t$ block samples of length $\beta k$ uniformly at random from the string $S$, and returns the sum of the sizes of the hitting sets divided by $t k \beta$. 
Recall that $\mathbb{E}[Y] = \mu$, where $(1-\tau) \epsilon \leq \mu \leq \epsilon$, so to get the desired approximation, it suffices to estimate $Y$
with an additive error of no more than $\delta$ with constant probability. Chebyshev inequality implies that it suffices to have $Var(Y) = \Theta(\delta^2)$. In other words, it will be enough to sample
$t = \Theta(\epsilon /k \delta^2)$ blocks, each of size $\beta k = \Theta(k / \tau)$. In total, it is enough to make $\Theta(k\epsilon (1/k-\epsilon) / \tau \delta^2) = O(\epsilon/\tau \delta^2)$ queries.

In the setting of approximation, $\epsilon$ is not known in advance, but $\epsilon \leq 1/k$ always holds,
so sampling $t = \Theta(1/k^2 \delta^2)$ blocks would suffice to get the desired additive error. 
The return value of the approximation algorithm will be its estimate of $Y$.
The query complexity and running time are $\beta t k = \Theta(1 / k \tau \delta^2)$.
This finishes the proof of Theorem \ref{thm:approx1D}.

%However, as $\epsilon$ is not known in advance in the setting of Theorem \ref{thm:approx1D}, we will need to make $O(1 / \tau \delta^2)$
%queries in this case to make sure that the additive error is small enough, finishing the proof of Theorem \ref{thm:approx1D}.
Now consider the setting of $(\epsilon_1, \epsilon_2)$-tolerant testing. 
By monotonicity of the tester, we can assume that we are given a string whose distance from $P$-freeness is either exactly $\epsilon_2$ or
exactly $\epsilon_1$.
Pick $\epsilon = \epsilon_2$, $\delta = (\epsilon_2 - \epsilon_1)/4$, $\tau = (\epsilon_2 - \epsilon_1) / 4 \epsilon_2$, 
and sample $t = \Theta(\epsilon /k \delta^2)$ blocks, with query complexity and running time
$\Theta(\epsilon /\tau \delta^2) = \Theta(\epsilon_2^2 / {\epsilon_2 - \epsilon_1}^3)$, as was stated above.
If the given string $S$ is $\epsilon_2$-far from $P$-freeness, then with probability at least $2/3$,
after sampling $t = \Theta(\epsilon /\tau \delta^2)$ samples, the value of $Y$ will be bigger than $(\epsilon_2)*(1 - \tau) - \delta = (\epsilon_2 + \epsilon_1)/2$.
On the other hand, if $S$ is $\epsilon$-close then with probability at least $2/3$, $Y \leq \epsilon_1 + \delta < (\epsilon_2 + \epsilon_1)/2$ 
Therefore, the tester will answer that the input is $\epsilon_2$-far if and only if $Y \geq (\epsilon_2 + \epsilon_1)/2$.
This finishes the proof of Theorem \ref{thm:test_1D}.


%The situation for tolerant testing (in Theorem \ref{thm:test_1D}) is quite different. Since we only need to distinguish between $\epsilon_1$-closeness
%and $\epsilon_2$-farness, we may take suitable $\delta = \Theta(\epsilon_2 - \epsilon_1)$ and $\tau = \Theta((\epsilon_2 - \epsilon_1) / \epsilon_2)$ with small enough constants,
%and make the number of queries that is needed to get an additive error of less than $\delta n$ with good probability,
%for an input whose distance from $P$-freeness is exactly $\epsilon = \epsilon_2$. Following the
%same steps as in the proof of Claim \ref{clm:approx_to_testing} in \cite{ParnasRonRubinfeld2006},
%and since the required number of queries increases with $\epsilon$,
%it is not hard to see that an $(\epsilon_1, \epsilon_2)$-tolerant tester is obtained, and that the number of queries and running time are $ O(\epsilon/\tau \delta^2) = O(\epsilon_2^2 / (\epsilon_2 - \epsilon_1)^3)$, as desired.
%
%
%by picking suitable $\delta = \Theta(\epsilon_2 - \epsilon_1)$ and $\tau = \Theta((\epsilon_2 - \epsilon_1) / \epsilon_2)$ in the
%statement of Theorem \ref{thm:approx1D}. The query complexity and the running time are $O(\epsilon_2^2 / (\epsilon_2 - \epsilon_1)^3)$.
\end{proof} 

